Leveraging Large Language Models for Effective Label-free Node Classification in Text-Attributed Graphs

Graph neural networks (GNNs) have become the preferred models for node classification in graph data due to their robust capabilities in integrating graph structures and attributes. However, these models heavily depend on a substantial amount of high-quality labeled data for training, which is often costly to obtain. With the rise of large language models (LLMs), a promising approach is to utilize their exceptional zero-shot capabilities and extensive knowledge for node labeling. Despite encouraging results, this approach either requires numerous queries to LLMs or suffers from reduced performance due to noisy labels generated by LLMs. To address these challenges, we introduce Locle, an active self-training framework that does Label-free node Classification with LLMs cost-Effectively. Locle iteratively identifies small sets of "critical" samples using GNNs and extracts informative pseudo-labels for them with both LLMs and GNNs, serving as additional supervision signals to enhance model training. Specifically, Locle comprises three key components: (i) an effective active node selection strategy for initial annotations; (ii) a careful sample selection scheme to identify "critical" nodes based on label disharmonicity and entropy; and (iii) a label refinement module that combines LLMs and GNNs with a rewired topology. Extensive experiments on five benchmark text-attributed graph datasets demonstrate that Locle significantly outperforms state-of-the-art methods under the same query budget to LLMs in terms of label-free node classification. Notably, on the DBLP dataset with 14.3k nodes, Locle achieves an 8.08% improvement in accuracy over the state-of-the-art at a cost of less than one cent. Our code is available at https://github.com/HKBU-LAGAS/Locle.

==> pictures/few_shot_cache.tex <==
\begin{table*}[!t]
\centering
\renewcommand{\arraystretch}{0.9}
\caption{Classification Performance.}\vspace{-3mm}
\begin{small}
\addtolength{\tabcolsep}{-0.25em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c c c c|c c c c|c c c c|c c c c|c c c c}
\hline
\multirow{2}{*}{\bf Backbone} & \multirow{2}{*}{\bf Method} & \multicolumn{4}{c|}{\bf{ {\em Cora}}} & \multicolumn{4}{c|}{\bf{ {\em CiteSeer}}} & \multicolumn{4}{c|}{\bf{ {\em PubMed}}} & \multicolumn{4}{c|}{\bf{ {\em WikiCS}}}  & \multicolumn{4}{c}{\bf{ {\em DBLP}}}  \\ \cline{3-22}

& & Acc & NMI & ARI & F1 & Acc & NMI & ARI & F1 & Acc & NMI & ARI & F1 & Acc & NMI & ARI & F1  & Acc & NMI & ARI & F1 \\ 
\hline
\multirow{3}{1cm}{\centering MLP\cite{}} & Base &&&&&&&&&&&&&&&&&&&&\\ 
 & LINK &&&&&&&&&&&&&&&&&&&&\\ 
  & LINKX &&&&&&&&&&&&&&&&&&&&\\ 
 \hline
\multirow{5}{1cm}{\centering Bert~\cite{devlin2019bertpretrainingdeepbidirectional}} &  Base &29.36&0.38&-0.19&7.86&19.27&0.44&0.28&11.58&20.83&0&0&19.15&7.71&1.61&0.43&9.88&18.41&0.20&-0.07&14.08 \\ 
& RoBERTa\cite{liu2019robertarobustlyoptimizedbert} &20.61&3.57&-0.24&15.00&18.20&1.55&1.12&14.58&23.5&1.87&-1.14&24.61&21.25&12.15&5.45&18.25&24.18&1.74&-0.27&20.74\\ 

& DistilBERT\cite{Sanh2019DistilBERTAD} &20.31&4.14&1.02&13.40&18.42&2.99&0.34&11.48&28.93&0.99&1.14&32.26&20.07&9.28&3.76&11.33&18.66&0.69&-0.4&20.21\\ 
& DistilRoBERTa &20.97&2.79&-0.71&13.74&25.17&8.21&4.33&22.08&38.31&4.39&4.04&30.20&28.10&17.44&8.57&28.16&18.03&2.56&0.75&17.61\\ 
& Sentence-Bert\cite{reimers2019sentencebertsentenceembeddingsusing} &56.20&35.68&32.84&54.06&45.35&30.19&26.1&44.51&32.71&14.08&1.02&42.51&59.95&37.52&32.75&57.16&55.84&23.11&16.89&55.75\\ 

\hline
\multirow{1}{1cm}{\centering Bart~\cite{lewis2019bartdenoisingsequencetosequencepretraining}} & 
 BART-Large-MNLI &40.88&16.62&12.44&39.07&42.81&16.7&14.66&38.29&67.60&29.37&29.42&66.64&46.69&24.51&19.61&43.28&49.06&8.79&9.46&44.67\\ 
 \hline
 \multirow{4}{1cm}{\centering Graph-LLM\cite{chen2024exploring}} & Zero-shot
     &67.00&-&-&-&65.50&-&-&-&90.75&-&-&-&&&&&&&& \\
     & Few-shot
     &67.75&-&-&-&66.00&-&-&-&85.50&-&-&-&&&&&&&& \\
     & Zero-Shot with 2-hop info
      &71.75&-&-&-&62.00&-&-&-&88.00&-&-&-&&&&&&&& \\
      & Few-shot with 2-hop info
      &74.00&-&-&-&67.00&-&-&-&79.25&-&-&-&&&&&&&&
      \\ 
\hline
\multirow{5}{1cm}{\centering GCN~\cite{kipf2016semi}} & SL-SD & 80.77 & 62.76 & 60.94 & 79.01 & 75.68 & 49.83 & 52.96 & 68.55 & 82.97 & 48.16 & 55.05 & 82.60 & &  &  &  &   73.45 & 40.64 & 45.94 & 66.69\\ 
& SL-random & &&&& &  &  &  & &  &  &  & & &  &  & 76.71 & 44.63 & 52.85 & 72.69 \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  &  &  & \\ 
& LLM-GNN+FP & 72.90 & 55.18 & 51.05 & 70.13 & 65.08 & 41.72 & 38.37 & 62.31 & 80.44 & 43.07 & 49.72 & 79.02 &  &  &  & & 67.43 & 38.78 & 34.96 & 66.22 \\ 
& LLM-GNN+gpart & 70.96 & 54.12& 49.45 &66.89 & 67.28 & 41.41 & 40.57 & 63.63 & 81.04 & 45.24 & 51.79 & 79.85 &  &  &  & & 73.28 & 40.97 & 46.31 & 68.54 \\ 
& LLM-GNN+rim &  72.14 & 53.50 & 52.36 & 69.04& 62.61 & 37.76 & 34.68 & 58.87 & 82.21 & 47.42 & 54.13 & 81.34 &  &  &  & & 67.72 & 36.97 & 34.02 & 67.15 \\ 
& LLM-GNN+SD & 75.56 & 55.68 & 56.31 &72.10 & 71.46 & 47.11 & 47.18 & 66.16 & 79.76 & 42.53 & 49.53 & 77.95 & 70 &  &  & & 67.21 & 38.83 & 34.44 & 66.18 \\ \cline{2-22}
& \algo & 80.10 & 63.95 & 62.04 & 74.75 & 75.34 & 49.57 & 52.73 & 66.80 & 82.23 & 47.13 & 53.67 & 81.81 & 72.65  & 53.81 & 54.62 & 66.24 & 76.56 & 45.03 & 51.38 & 73.67\\ 
& Improv. &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & &  &  & & \\ 
\hline 
\multirow{5}{1cm}{\centering GAT~\cite{velivckovic2017graph}} & SL-SD & 80.43& 61.56 & 60.17 & 79.31& 73.28 & 48.07 & 49.40 & 68.95 & 76.32 & 36.58 & 40.53 & 76.57 &  &  &  & & 61.82 & 34.03& 36.33 &55.53\\ 
% \multirow{5}{1cm}{\centering GAT~\cite{}} & SL-SD & 72.03 & 39.33& 44.21 &65.36 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & SL-random &65.44&33.15&31.91&58.26& &  &  &  & &  &  &  & & &  &  & \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+FP & 57.98& 31.26 & 25.24 & 55.76 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+gpart & 61.49& 33.31& 31.35 & 60.05 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+rim & 59.19 & 33.99 & 24.34 & 60.13 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+SD & 64.33 & 35.74 & 32.68 & 62.43 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & \algo & & &  & &  &  &  &  &  &  &  & &  &  &  & &  \\ 
& SL-random & &&&& &  &  &  & 81.55 & 44.84 & 51.74 & 81.19 & & &  &  & 68.59&37.51&37.99&56.54 \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  &  &  & \\ 
& LLM-GNN+FP & 69.11 & 48.83 & 44.14 & 66.36 & 60.97 & 39.44 & 36.01 & 56.88 & 77.10 & 36.93 & 43.51 & 75.06 &  &  &  & & 68.64& 39.76 & 40.28 & 66.99 \\ 
& LLM-GNN+gpart &69.63 & 48.35& 46.75 &65.91 & 62.25 & 38.22 & 33.35 & 56.84 & 77.40& 38.59 & 45.65 & 74.77 & 56.01 &  &  & & 66.47& 36.09& 33.55 & 65.53\\ 
& LLM-GNN+rim & 67.64  & 46.45& 44.14 & 65.22& 64.38 & 39.49 & 37.68 & 60.86 & 80.66 & 44.29 & 50.72 & 79.39 &  &  &  & & 59.19 & 33.99 & 24.34 & 60.13 \\ 
& LLM-GNN+SD & 70.17 & 48.84& 47.86 &67.07 & 69.67 & 45.61 & 43.64 & 64.71 & 76.31 & 38.73 & 41.89 & 75.80 &  &  &  & & 65.85 & 35.39 & 34.66 & 62.84\\ \cline{2-22}
& \algo & 75.28 & 55.35 & 54.13 & 72.62 & 72.76 & 46.30 & 48.57 & 62.14 & 81.68 & 45.23 & 52.04 & 81.32 &  &  &  & & 75.06 & 41.75 & 48.28 & 71.50 \\ 
& Improv. &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & &  &  & & \\ 
\hline
% \multirow{5}{1cm}{\centering GCNII~\cite{}} & SL-SD & 63.19 & 29.79 & 32.69 & 50.16 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & SL-random & 76.07& 44.30& 51.15& 72.94& &  &  &  & &  &  &  & & &  &  & \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+FP & 68.68 & 39.68 & 37.78 & 67.58 &  &  &  &  &  &  &  & &  &  &  & & \\ 
% & LLM-GNN+gpart & 70.08 & 41.43 & 51.28 & 71.98 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+rim & 68.89 & 39.45 & 36.25 & 68.25 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+SD & 62.38& 33.51& 29.37 & 53.93 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & \algo & 75.67 & 43.46 & 51.36 & 69.13 &  &  &  &  &  &  &  & &  &  &  & & \\ 
% \hline
\multirow{5}{1cm}{\centering GCNII~\cite{chen2020simple}} & SL & 80.73& 60.37 & 62.32& 78.64 & 59.44 & 39.48 & 34.31 & 57.96 & 81.88 & 44.60 & 52.97 & 81.03 &  &  &  & &   63.19 & 29.79 & 32.69 & 50.16 \\ 
& SL-random & &&&& 69.43 & 42.21 & 43.48 & 65.74 & &  &  &  & & &  &  & 76.07& 44.30& 51.15& 72.94 \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  &  &  & \\ 
& LLM-GNN+FP & 70.14 & 50.21& 45.53 &67.52 & 59.81 & 35.60 & 31.22 & 57.07 & 77.03 & 36.56 & 44.52 & 74.21 &  &  &  & & 68.68 & 39.68 & 37.78 & 67.58 \\ 
& LLM-GNN+gpart &70.88 & 49.95& 48.57 &66.91 & 63.81 & 38.07 & 35.88 & 60.52 & 79.46 & 41.11 & 49.54 & 77.38 &  &  &  & & 70.08 & 41.43 & 51.28 & 71.98 \\ 
& LLM-GNN+rim &69.05 & 48.92 & 46.66 & 66.16& 62.44 & 38.79 & 36.79 & 59.36 & 78.57 & 40.62 & 48.29 & 75.48 &  &  &  & &68.89 & 39.45 & 36.25 & 68.25 \\ 
& LLM-GNN+SD & 70.36  & 50.33 & 49.53 &64.14 &  56.83 & 34.18 & 29.41 & 53.95 & 77.23 & 37.30 & 45.47 & 74.48 &  &  &  & &   62.38& 33.51& 29.37 & 53.9\\ \cline{2-22}
& \algo & 75.98 & 57.62 & 56.97 & 71.95 & 70.87 & 44.05 & 45.19 & 62.81 & 81.46 & 44.97 & 51.96 & 80.88 &  &  &  & & 75.67 & 43.46 & 51.36 & 69.13\\ 
& Improv. &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & &  &  & & \\ 
\hline
\end{tabular}
}
\end{small}
\label{tbl:quality}
\vspace{-2mm}
\end{table*}

==> pictures/hyper_param_selection.tex <==


% Table 2
\begin{table}[ht]
\centering
\caption{Hyperparameters for GatedGCN+VN.}
\begin{tabular}{lcccccc}
\toprule
 & PascalVOC-SP & COCO-SP & Peptides-Func & Peptides-Struct & ogbg-code2 & ogbg-molpcba \\
\midrule
lr & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 & 0.001 \\
dropout & 0.1 & 0.1 & 0.1 & 0.1 & 0.3 & 0.4 \\
\#layers & 10 & 6 & 8 & 10 & 5 & 6 \\
hidden dim. & 70 & 90 & 80 & 70 & 256 & 1024 \\
head depth & 2 & 1 & 2 & 2 & 1 & 1 \\
PE/SE & none & none & RWSE & LapPE & none & RWSE \\
VN pooling & mean & mean & mean & mean & mean & sum \\
batch size & 50 & 50 & 200 & 200 & 32 & 512 \\
\#epochs & 200 & 200 & 250 & 250 & 50 & 60 \\
\#Param. & 478K & 453K & 486K & 466K & 1.20M & 57M \\
time/epoch & 66s & 206s & 24s & 28s & 502s & 487s \\
\bottomrule
\end{tabular}
\label{tbl:gcn_param_selection}
\end{table}

% Table 3
\begin{table}[ht]
\centering
\caption{Hyperparameters for GCN+VN.}
\begin{tabular}{lccccc}
\toprule
 & PascalVOC-SP & COCO-SP & Peptides-Func & Peptides-Struct \\
\midrule
lr & 0.001 & 0.001 & 0.001 & 0.001 \\
dropout & 0.2 & 0.1 & 0.1 & 0.1 \\
\#layers & 8 & 10 & 10 & 8 \\
hidden dim. & 105 & 95 & 95 & 105 \\
head depth & 2 & 3 & 3 & 2 \\
PE/SE & none & none & RWSE & LapPE \\
VN pooling & mean & mean & mean & mean \\
batch size & 50 & 50 & 200 & 200 \\
\#epochs & 200 & 200 & 250 & 250 \\
\#Param. & 460K & 465K & 487K & 474K \\
time/epoch & 35s & 156s & 18s & 19s \\
\bottomrule
\end{tabular}
\end{table}




==> pictures/quality.tex <==
\begin{table*}[!t]
\centering
\renewcommand{\arraystretch}{0.9}
\caption{Classification Performance.}\vspace{-3mm}
\begin{small}
\addtolength{\tabcolsep}{-0.25em}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|c c c c|c c c c|c c c c|c c c c|c c c c}
\hline
\multirow{2}{*}{\bf Backbone} & \multirow{2}{*}{\bf Method} & \multicolumn{4}{c|}{\bf{ {\em Cora}}} & \multicolumn{4}{c|}{\bf{ {\em CiteSeer}}} & \multicolumn{4}{c|}{\bf{ {\em PubMed}}} & \multicolumn{4}{c|}{\bf{ {\em WikiCS}}}  & \multicolumn{4}{c}{\bf{ {\em DBLP}}}  \\ \cline{3-22}
& & Acc & NMI & ARI & F1 & Acc & NMI & ARI & F1 & Acc & NMI & ARI & F1 & Acc & NMI & ARI & F1  & Acc & NMI & ARI & F1 \\ \hline
\multirow{3}{1cm}{\centering MLP} & Base &63.53&40.39&38.19&58.68&61.04&36.50&31.95&58.36&76.62&36.86&41.82&74.38&60.72&39.72&38.79&55.22&60.37&24.80&23.19&59.66 \\ 
& LINK~\cite{lim2021largescalelearningnonhomophilous} &43.36&26.02&11.69&43.33&30.60&13.28&1.81&23.97&48.19&6.30&2.45&36.46&50.95&32.91&24.24&46.45&29.50&7.41&2.64&31.07 \\
& LINKX ~\cite{lim2021largescalelearningnonhomophilous} &59.02&41.27&31.98&56.59&62.49&35.84&33.71&58.61&65.64&24.37&23.21&58.86&42.95&31.87&20.36&33.59&45.05&13.60&11.31&42.85 \\ \hline
\multirow{5}{1cm}{\centering Bert~\cite{devlin2019bertpretrainingdeepbidirectional}} &  Base &29.36&0.38&-0.19&7.86&19.27&0.44&0.28&11.58&20.83&0&0&19.15&7.71&1.61&0.43&9.88&18.41&0.20&-0.07&14.08 \\ 
& RoBERTa~\cite{liu2019robertarobustlyoptimizedbert} &20.61&3.57&-0.24&15.00&18.20&1.55&1.12&14.58&23.5&1.87&-1.14&24.61&21.25&12.15&5.45&18.25&24.18&1.74&-0.27&20.74\\ 
& DistilBERT~\cite{Sanh2019DistilBERTAD} &20.31&4.14&1.02&13.40&18.42&2.99&0.34&11.48&28.93&0.99&1.14&32.26&20.07&9.28&3.76&11.33&18.66&0.69&-0.4&20.21\\ 
& DistilRoBERTa &20.97&2.79&-0.71&13.74&25.17&8.21&4.33&22.08&38.31&4.39&4.04&30.20&28.10&17.44&8.57&28.16&18.03&2.56&0.75&17.61\\ 
& Sentence-Bert~\cite{reimers2019sentencebertsentenceembeddingsusing} &56.20&35.68&32.84&54.06&45.35&30.19&26.1&44.51&32.71&14.08&1.02&42.51&59.95&37.52&32.75&57.16&55.84&23.11&16.89&55.75\\  \hline
\multirow{1}{1cm}{\centering Bart~\cite{lewis2019bartdenoisingsequencetosequencepretraining}} & 
 BART-Large-MNLI &40.88&16.62&12.44&39.07&42.81&16.7&14.66&38.29&67.60&29.37&29.42&66.64&46.69&24.51&19.61&43.28&49.06&8.79&9.46&44.67\\ 
 \hline
 \multirow{2}{1cm}{\centering Graph-LLM~\cite{chen2024exploring}} 
 & Zero-shot  
     &64.00&45.47&38.03&- &63.00&42.66&35.91&-&86.00&59.51&65.78&83.35&66.00&57.21&47.42&-&64.00&30.10&31.56&- \\
     & Zero-shot (COT)
     &68.00&46.38&40.22&-&65.50&46.18&37.35&-&83.00&56.02&61.21&-&65.50&53.65&47.72&-&67.50&31.61&34.42&- \\
     & Zero-Shot (2-Hop)
      &72.00&56.02&47.72&-&59.50&41.87&32.35&-&86.50&60.39&66.70&-&64.50&51.40&42.25&-&76.50&45.72&48.13&- \\ \hline
\multirow{5}{1cm}{\centering GCN~\cite{kipf2016semi}}  & LLM-GNN+FP & 72.52 & 54.83 & 52.56 & 68.77 &66.81&44.46&40.23&63.88&79.90&42.44&48.79&77.97&65.75&51.06&47.34&54.43&70.19&38.06&38.48&69.00 \\ 
& LLM-GNN+gpart &71.20&53.88&48.67&67.76&70.86&46.20&46.00&66.04&81.97&45.70&52.97&80.92&66.26&50.51&48.57&58.21&70.53&37.29&39.46&68.90 \\  & LLM-GNN+rim &72.34&52.46&52.47&68.55&66.51&42.15&39.09&62.63&82.41&46.62&55.08&81.21&66.44&49.50&46.87&54.74&73.15&42.16&43.69&71.81 \\ 
% & LLM-GNN+SD  &76.11&56.65&58.05&71.73&66.95&42.91&40.24&63.02&82.06&45.71&53.09&81.14&71.29&52.01&53.44&63.45&70.15&40.58&41.49&68.29 \\
\cline{2-22}
& \algo &\cellcolor{gray!30} 81.80&\cellcolor{gray!30} 64.22&64.30&79.64&76.16&50.87&54.14&65.28&83.70&48.86&56.56&83.26&75.23&55.18&58.98&69.54&75.55&44.33&49.43&73.38\\ 
& Improv. & 9.28 & 9.39 & 11.74 & 10.87 & 5.30 & 4.67 & 8.14 & -0.76 & 1.29 & 2.24 & 1.48 & 2.05 & 8.08 & 3.09 & 8.80 & 11.08 & 2.40 & 2.17 & 5.74 & 1.57 \\

 \hline 
\multirow{5}{1cm}{\centering GAT~\cite{velivckovic2017graph}}  & LLM-GNN+FP & 68.78 & 47.30 & 44.65 & 65.52&60.58&38.56&33.02&57.92&80.76&42.94&50.56&79.37&67.36&48.87&47.07&62.73&69.51&37.01&37.67&67.76 \\ 
& LLM-GNN+gpart &69.05&48.34&44.63&66.13&67.76&41.80&41.42&63.86&81.65&44.80&52.44&80.49&64.36&45.91&43.46&59.30&66.01&33.48&34.00&63.44\\ 
& LLM-GNN+rim &66.19&44.86&42.84&63.29&64.10&40.02&37.38&60.68&82.47&46.64&54.53&81.41&66.85&47.51&46.12&61.97&68.76&38.08&36.80&67.46 \\  \cline{2-22}
& \algo &76.06&56.75&55.78&73.24&73.97&47.38&50.27&66.26&82.48&46.08&53.94&81.94&73.23&54.22&54.83&67.80&76.37&44.14&50.75&74.12 \\ 
& Improv. & 7.01 & 8.41 & 11.13 & 7.11 & 6.21 & 5.58 & 8.85 & 2.40 & 0.01 & -0.56 & -0.59 & 0.53 & 5.87 & 5.35 & 7.76 & 5.07 & 6.86 & 6.06 & 13.08 & 6.36 \\  \hline
\multirow{5}{1cm}{\centering GCNII~\cite{chen2020simple}} & LLM-GNN+FP & 69.37 & 49.12& 45.98 &65.73 &60.23&36.38&32.17&57.80&77.79&38.54&45.05&75.30&60.77&45.47&39.94&53.45&73.88&42.73&45.20&72.53 \\ 
& LLM-GNN+gpart &70.28&50.56&47.52&66.71&63.55&37.82&35.31&59.89&80.78&43.01&51.47&79.05&57.47&41.00&37.92&47.85&69.54&38.36&37.68&68.56 \\ 
& LLM-GNN+rim &69.52&49.01&47.75&65.85&65.04&40.26&38.48&61.63&79.81&42.47&50.60&77.14&64.90&46.22&43.44&59.08&66.72&39.13&33.92&66.41 \\  \cline{2-22}
& \algo &78.71&58.76&58.45&76.81&73.14&47.19&49.28&65.45&82.08&45.58&53.44&81.37&68.70&49.48&50.53&62.11&75.23&43.38&48.60&72.59\\ 
& Improv. & 8.43 & 8.20 & 10.70 & 10.10 & 8.10 & 6.93 & 10.80 & 3.82 & 1.30 & 2.57 & 1.97 & 2.32 & 3.80 & 3.26 & 7.09 & 3.03 & 1.35 & 0.65 & 3.40 & 0.06 \\ 
\hline


\end{tabular}
}
\end{small}
\label{tbl:quality}
\vspace{-2mm}
\end{table*}

% \begin{table*}[!t]
% \centering
% \renewcommand{\arraystretch}{1.0}
% \caption{Classification Performance.}\vspace{-3mm}
% \begin{small}
% \addtolength{\tabcolsep}{-0.25em}
% % \resizebox{\textwidth}{!}{%
% \begin{tabular}{c|c|c c c c|c c c c|c c c c|c c c c|c}
% \hline
% \multirow{2}{*}{\bf Backbone} & \multirow{2}{*}{\bf Method} & \multicolumn{4}{c|}{\bf{ {\em DBLP}}} & \multicolumn{4}{c|}{\bf{ {\em Arxiv}}} & \multicolumn{4}{c|}{\bf{ {\em XXX}}} & \multicolumn{4}{c|}{\bf{ {\em XXX}}}  & \multirow{2}{*}{\bf Rank}  \\ \cline{3-18}

% & & Acc & F1 & NMI & ARI & Acc & F1 & NMI & ARI & Acc & F1 & NMI & ARI & Acc & F1 & NMI & ARI  & \\ 
% \hline
% \multirow{5}{1cm}{\centering GCN~\cite{}} & SL-SD & 73.45 & 40.64 & 45.94 & 66.69 &  &  &  &  & &  &  &  & & &  &  & \\ 
% & SL-random & 76.71 & 44.63 & 52.85 & 72.69 & &  &  &  & &  &  &  & & &  &  & \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+FP & 67.43 & 38.78 & 34.96 & 66.22 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+gpart & 73.28 & 40.97 & 46.31 & 68.54 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+rim & 67.72 & 36.97 & 34.02 & 67.15 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+SD & 67.21 & 38.83 & 34.44 & 66.18 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & \algo & 76.56 & 45.03 & 51.38 & 73.67 &  &  &  &  &  &  &  & &   &  &  & &  \\ 
% \hline
% \multirow{5}{1cm}{\centering GAT~\cite{}} & SL-SD & 72.03 & 39.33& 44.21 &65.36 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & SL-random &65.44&33.15&31.91&58.26& &  &  &  & &  &  &  & & &  &  & \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+FP & 57.98& 31.26 & 25.24 & 55.76 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+gpart & 61.49& 33.31& 31.35 & 60.05 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+rim & 59.19 & 33.99 & 24.34 & 60.13 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+SD & 64.33 & 35.74 & 32.68 & 62.43 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & \algo & & &  & &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% \hline
% \multirow{5}{1cm}{\centering GCNII~\cite{}} & SL-SD & 63.19 & 29.79 & 32.69 & 50.16 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & SL-random & 76.07& 44.30& 51.15& 72.94& &  &  &  & &  &  &  & & &  &  & \\ 
% & Graph-LLM & & &  & &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+FP & 68.68 & 39.68 & 37.78 & 67.58 &  &  &  &  &  &  &  & &  &  &  & & \\ 
% & LLM-GNN+gpart & 70.08 & 41.43 & 51.28 & 71.98 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+rim & 68.89 & 39.45 & 36.25 & 68.25 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & LLM-GNN+SD & 62.38& 33.51& 29.37 & 53.93 &  &  &  &  &  &  &  & &  &  &  & &  \\ 
% & \algo & 75.67 & 43.46 & 51.36 & 69.13 &  &  &  &  &  &  &  & &  &  &  & & \\ 
% \hline
% \end{tabular}
% % }
% \end{small}
% \label{tbl:quality}
% \vspace{-2mm}
% \end{table*}

==> tex/method.tex <==
\section{Methodology}

% \subsection{LM-based Text Embeddings}
% Use BERT or Sentence-BERT to get node initial embeddings

% \subsection{Graph Neural Networks}

% Use GNN to get node embeddings

% \subsection{Clustering Module}

% Use Embedding to get node-cluster indicator, i.e., centroid embeddings

\subsection{LLMs}

\begin{enumerate}
\item Use BERT or Sentence-BERT to get node initial embeddings $\HM^{(0)}$
\item Sample a subset of nodes (\renchi{use top-$k$ PageRank to select $k$ nodes or use $k$-Means over the node initial embeddings to get the $k$ centroids}) from different regions of the graph. Use LLMs to label nodes, and create pseudo labels $\mathcal{Y}$. \url{https://arxiv.org/pdf/2310.04668}
\item With $\HM^{(0)}$ and pseudo labels $\mathcal{Y}$, train GNN models (use GCN, APPNP, GCNII, and GAT as backbones) to get node embeddings $\HM$ and predict node-label predictions $\mathbf{Y}$.
\item Use LLMs to correct misclustering in $\mathbf{Y}$ and get hard positive/negative samples.
\item Update the graph structure $\AM$ according to hard positive/negative samples and update node labels $\mathcal{Y}$ accordingly. Retrain the GNN model.
\end{enumerate} 

\subsection{Ensemble Clustering}
Let $\YM^{(\ell)}$ be the node-cluster indicator matrix obtained at $\ell$-th round.
Every $L$ rounds, we enter into a phase correcting the misclustering.
Let $\YM = \sum_{\ell=1}^{L}{w_\ell\YM^{(\ell)}}$ be the ensemble clustering result, where $w_\ell$ can be $\frac{1}{L}$ or others.
\renchi{$w_\ell = \frac{(1-\alpha)\alpha^{L-\ell}}{1-\alpha^{L}}$}
We can compare $\YM$ and the ground-truth labels to observe the patterns of correctly labeled nodes and incorrectly labeled nodes in $\YM$. The goal is to leverage the patterns to design a function to mark incorrectly labeled nodes as unconfident samples and correctly labeled nodes as confident samples.
Need to define a measure to evaluate the confidence.

In confident samples, nodes with the same labels should be connected in $\AM$. Nodes with different labels should be disconnected in $\AM$. This step is to add homophily connections and remove heterophily connections.

For unconfident samples, find those with the lowest confidence, denoted as $\mathcal{U}$. Suppose for each label we have some representative confident samples $\mathcal{C}$. For each $v$ sample in $\mathcal{U}$, we can ask LLM $v$ is close to which samples in $\mathcal{C}$ and assign the corresponding label to $v$ to correct its label. This step is to inject the knowledge of LLMs to facilitate labeling the nodes that the GNNs cannot handle merely based on the model and current knowledge.

Another way is to utilize the co-association matrix to get these confident or unconfident samples.
See the co-association matrix defined in the related work section in \url{https://ojs.aaai.org/index.php/AAAI/article/view/29552/30923}.

\renchi{Do a sanity check: For unconfident nodes, may check their neighbors' labels and their labels to see if the differences are large. If yes, we need to rely more on LLMs. If not, GNN may be more helpful (seems that in this case, labels of these nodes are easier to infer and will not become unconfident nodes). May also check if the labels of them and their most similar nodes in confident node set (in terms of textual contents/embeddings) are the same. If so, it means that confident nodes with similar embeddings/textual contents can help us infer the labels of the unconfident nodes. Then, we need to select representative confident nodes input to LLMs according to their similarities to unconfident nodes other than randomly select.}

\renchi{Read: \url{https://arxiv.org/pdf/2305.14871} and \url{https://arxiv.org/pdf/2307.00524} for other LLM-based clustering methods.}

\renchi{As for theory, we may refer to \url{https://arxiv.org/pdf/1706.07510}, \url{https://proceedings.neurips.cc/paper_files/paper/2017/file/db5cea26ca37aa09e5365f3e7f5dd9eb-Paper.pdf} and \url{https://papers.nips.cc/paper_files/paper/2016/file/9597353e41e6957b5e7aa79214fcb256-Paper.pdf}, \url{https://proceedings.mlr.press/v162/xia22a/xia22a.pdf}, \url{https://arxiv.org/abs/2002.11557}, \url{https://arxiv.org/abs/2402.01400} when regarding LLM or GNN as the oracle.}


\section{Overall Framework}

Basic idea: Call LLMs only for a few nodes. Use GNNs or other cheap models to handle the majority of nodes.

\subsection{Preliminary Node Annotation}

\begin{itemize}
    \item Which nodes (denoted as set $\Sc$) and how many nodes should be selected from $\V$?
    \item How do we ask LLMs properly to get the labels of nodes in $\Sc$?
\begin{itemize}
    \item if label texts are given (zero-shot classification, see \cite{li2023prompt})
    \item if label texts are unknown (clustering)
\end{itemize}
\end{itemize}

% May borrow some ideas from active learning \cite{huang2024cost}.

\renchi{
Node feature representations:
\begin{equation}
\ZM = \sum_{t=0}^{T}{\alpha^t \NAM^t \XM},
\end{equation}
where $\NAM$ is the normalized adjacency matrix and $\XM$ is the ($L_2$ normalized or original) node attribute matrix. It's the optimal solution to the Graph Laplacian Smoothing problem (see Definition 3.1 in \url{https://arxiv.org/pdf/2403.13268}, Section 3.2 in \url{https://arxiv.org/pdf/2110.11842}, and Lemma 1 in \url{https://arxiv.org/pdf/2401.09071}).

Use the subspace clustering method, whose objective function is:
\begin{equation}
    \min_{\SM\in \mathbb{R}^{n\times n}}{\|\ZM-\SM\ZM\|_F^2 + \Omega(\SM)}
\end{equation}
$\SM$ is the target self-representation or coefficient matrix, where $\SM_{i,j}$ denotes the affinity between nodes $v_i$ and $v_j$.

Read \url{https://chakib401.github.io/assets/pdf/SAGSC.pdf} to understand what is subspace clustering.

$\SM=\UM\UM^{\top}$ where $\UM$ is the $|\Sc|$ largest eigenvectors of $\ZM$. Apply K-Medoids or K-Center over $\UM$ to get the $|\Sc|$ centroids as $\Sc$, i.e., the nodes selected for labeling.
}


\subsection{Node Label Prediction}

use various GNN models to generate node-label predictions $\YM^{(\ell)}\in \mathbb{R}^{n\times k}$ at $\ell$-th round.

\subsection{Node Label and Structure Correction}

Use the idea of the ensemble clustering, we can assemble $L$ rounds results as $\YM$.

\begin{itemize}
    \item By $\YM$, how to categorize nodes into confident nodes, and unconfident nodes?
    \begin{itemize}
        \item For confident nodes, how to make use of them to revise the graph structure (add edges, remove edges) and correct wrong labels for $\Sc$ and create additional labelled data added to $\Sc$?
        \item For unconfident nodes, which nodes should be sent to LLMs and how do we ask LLMs properly to correct their predictions?
    \end{itemize}
\end{itemize}


Let $\LM = \DM-\AM$ be the Laplacian of the graph $\G$.

The {\em Dirichlet energy} (see \url{https://papers.nips.cc/paper_files/paper/2023/file/4d689f0f30199661a10aa2200488aebb-Paper-Conference.pdf}) of $\YM$ on $\G$ is
\begin{equation}
\YM_{\cdot,\ell}^\top\LM \YM_{\cdot,\ell} = \frac{1}{2}\sum_{(v_i,v_j)\in E}{(\YM_{i,\ell}-\YM_{j,\ell})^2},
\end{equation}
and if we consider all classes, we have
\begin{equation}\label{eq:obj-de}
trace(\YM^\top\LM \YM) = \frac{1}{2}\sum_{\ell=1}^k\sum_{(v_i,v_j)\in E}{(\YM_{i,\ell}-\YM_{j,\ell})^2}.
\end{equation}

Our goal is to update $\YM$ and rewire $\G$ such that Eq.~\eqref{eq:obj-de} is minimized. 
We can do empirical studies on real datasets to show the values in Eq.~\eqref{eq:obj-de} as the motivation. A high value means (i) the nodes are assigned the wrong predicted labels and (ii) edges connecting nodes from different ground-truth classes. 
The second issue may aggravate the first one due to the message passing paradigm in GNNs.

For the first issue, we can use LLM to alleviate. 
For the second one, we can use graph rewiring techniques.

\subsubsection{Identifying Confident/Unconfident Nodes}


\begin{definition}[Harmonicity]
Let $\YM$ be a $n\times k$ node-class predictions, where $\YM_{i,j}$ denotes the probability of node $v_i$ belonging to class $C_\ell$. Let $\tilde{\LM} = \IM-\DM^{-1}\AM$ be the random walk normalized Laplacian of graph $\G$. The harmonicity vector of nodes in $\G$ class $C_\ell$ is
\begin{equation}
\mathbf{h}^{(\ell)}_i = (\YM_{i,\ell} - \frac{1}{d(v_i)}\sum_{v_j\in N(v_i)}{\YM_{j,\ell}})^2 = (\tilde{\LM}\YM_{\cdot,\ell})^{\odot 2}_i
\end{equation}
The overall harmonicity w.r.t. all the $k$ classes is
\begin{equation}
 \mathbf{h} = (\sum_{\ell=1}^{k}{\mathbf{h}^{(\ell)}})^{\odot -\frac{1}{2}} = ((\tilde{\LM}\YM)^{\odot 2}\mathbf{1}_{k\times 1})^{\odot -\frac{1}{2}}.
\end{equation}
\end{definition}

Intuitively, $\mathbf{h}_i$ measures the degree of the difference of $v_i$'s labels from those of its neighbors. 
This notion is closely related to the local variation in \url{https://www.gretsi.fr/peyresq14/documents/1-Vandergheynst.pdf} used to measure how smooth $\YM$ is on $\G$ or the harmonic loss in \url{https://www4.comp.polyu.edu.hk/~csxmwu/papers/NIPS-2013-Harmonic.pdf}.

Next, we measure the distribution of probabilities in $\YM_{i,\cdot}\ \forall{v_i\in \V}$. We can use {\em entropy} to measure this
\begin{equation}
f(v_i) = \sum_{\ell=1}^k{\YM_{i,\ell}\cdot \log{\YM_{i,\ell}}}.
\end{equation}
When $\YM_{i,\cdot}$ is a even distribution, $f(v_i)$ attains the highest value.

Four cases:
\begin{itemize}
\item The node $v_i$ has a high harmonicity $\mathbf{h}_i$ and high classification prediction entropy $f(v_i)$, we are very unconfident about $v_i$'s label.
\item The node has a high harmonicity $\mathbf{h}_i$ but high classification prediction entropy $f(v_i)$, we are partially confident about $v_i$'s label but unconfident about $v_i$'s neighbors' labels or their edges.
\item The node has a low harmonicity $\mathbf{h}_i$ but low classification prediction entropy $f(v_i)$,  we are very confident about $v_i$'s label.
\item The node has a low harmonicity $\mathbf{h}_i$ and high classification prediction entropy $f(v_i)$, ?
\end{itemize}

% Simply, we need to find the unconfident nodes $\U$ with the $|\U|$ largest harmonicity scores.

% For nodes $v_i$ in $\U$, if the distribution of $\YM_{i,\cdot}$ is even, we are not confident about which classes this node should be assigned to, but if the distribution of $\YM_{i,\cdot}$ is biased, it means the model is confident on the classification. Need to take this into consideration before sending $\U$ to LLM.
% This implies that the neighbors of $v_i$ might be wrongly classified or the edges incident to $v_i$ are noisy. We should remove edges connecting two nodes assigned to different classes with high predictive scores.

\subsubsection{Adding and Removing Edges}

To minimize Eq.~\eqref{eq:obj-de}, we can rewire the topology of $\G$ to remove noisy edges and add shortcut edges.

Node pairs with low harmonicity and low classification prediction entropy and belong to the same class. Add links.



==> tex/methodology/GNN-labelling.tex <==
\subsection{Multi-Round Filter-Refinement}
We launch $R$ rounds of training, in which each round 

Initially, $\A$ serves as training set $\VTR$ and $\V\setminus \VTR$ serves as test set.

% In each $r$-th round, we 

filter-refinement paradigm

active learning and self-training

\subsubsection{\bf Sample Filtering}

This component aims to filter out $\VCS$ and $\VUS$ ($|\VUS| = \BLC/R$) from $\V\setminus \VTR$, referred to as {\em confident node set} and {\em unconfident node set}, i.e., bottleneck

\begin{equation}
\YM^{(\text{base})} = \textsf{GNN}(\G, \XM),
\end{equation}

We define label harmonicity and label entropy, which measure the {\em uncertainty} of the predictions of each node from the perspectives of samples and classes, i.e., rows and columns of $\YM^{(\text{base})}$.

We define the notion {\em label harmonicity} of a node $v_i\in \V\setminus \VTR$ as
\begin{definition}[Label Harmonicity]
\begin{footnotesize}
\begin{equation}
LH(v_i) = \sqrt{\sum_{j=1}^{k}{\left(\YM^{(\text{base})}_{i,j}-\frac{1}{|\N(v_i)|}\sum_{v_{\ell}\in \N(v_i)}{\YM^{(\text{base})}_{\ell,j}}\right)^2}}
\end{equation}
\end{footnotesize}
\end{definition}
whose matrix form can be represented by $((\tilde{\LM}\YM^{(\text{base})})^{\odot 2}\mathbf{1}_{k\times 1})^{\odot \frac{1}{2}}$.

Intuitively, $LH(v_i)$ measures the discrepancy of $v_i$'s class labels from those of its neighbors in $\G$. The larger $LH(v_i)$ is, the more unreliable the predicted labels of $v_i$ by $\YM^{(\text{base})}$ are.
% This notion is closely related to the local variation in \url{https://www.gretsi.fr/peyresq14/documents/1-Vandergheynst.pdf} used to measure how smooth $\YM$ is on $\G$ or the harmonic loss in \url{https://www4.comp.polyu.edu.hk/~csxmwu/papers/NIPS-2013-Harmonic.pdf}.

Additionally, we define the {\em label entropy} of a node $v_i\in \V\setminus \VTR$ as
\begin{definition}[Label Entropy]
\begin{small}
\begin{equation}
LE(v_i) = -\sum_{j=1}^{k} \YM^{(\text{base})}_{i,j} \cdot \log \left( \YM^{(\text{base})}_{i,j} + \varepsilon \right),
\end{equation}
\end{small}
\end{definition}\taiyan{not two $\YM^{(\text{base})}_{i,j}$}
where $\varepsilon$ (typically $10^{-9}$) is introduced to avoid zero values. 
A high label entropy value suggests that the predicted probabilities are evenly distributed among the possible classes, and hence, indicates that the prediction is highly uncertain.
Intuitively, the larger $LE(v_i)$ is, the less confident we are about the predictions.
% $\YM^{(\text{base})}_{i}$ is a even distribution, $LE(v_i)$ attains the highest value.

top $|\VUS|$ 
\begin{equation}
\Sset_{\text{har}} = \argtopk{v_i\in \V\setminus \VTR}{LH(v_i)}\ \text{and}\ \Sset_{\text{ent}} = \argtopk{v_i\in \V\setminus \VTR}{LE(v_i)}
\end{equation}

\begin{equation}
\VUS = \left( \Sset_{\text{har}} \cap \Sset_{\text{ent}} \right) \cup \left( \Sset_{\text{har}} \cap \Sset_{\text{ent}} \right)^{\complement}
\end{equation}
\renchi{How to choose $|\VUS|-|\Sset_{\text{har}} \cap 
\Sset_{\text{ent}}|$ nodes from $\left( \Sset_{\text{har}} \cap \Sset_{\text{ent}} \right)^{\complement}$?}
\taiyan{Choose $\frac{top(rank_{har}}{2})$ and $\frac{top(rank_{ent}}{2})$. }
% \begin{definition}[Harmonicity]
% Let $\YM$ be a $n\times k$ node-class predictions, where $\YM_{i,j}$ denotes the probability of node $v_i$ belonging to class $C_\ell$. Let $\tilde{\LM} = \IM-\DM^{-1}\AM$ be the random walk normalized Laplacian of graph $\G$. The harmonicity vector of nodes in $\G$ class $C_\ell$ is
% \begin{equation}
% \mathbf{h}^{(\ell)}_i = (\YM_{i,\ell} - \frac{1}{d(v_i)}\sum_{v_j\in N(v_i)}{\YM_{j,\ell}})^2 = (\tilde{\LM}\YM_{\cdot,\ell})^{\odot 2}_i
% \end{equation}
% The overall harmonicity w.r.t. all the $k$ classes is
% \begin{equation}
%  \mathbf{h} = (\sum_{\ell=1}^{k}{\mathbf{h}^{(\ell)}})^{\odot -\frac{1}{2}} = ((\tilde{\LM}\YM)^{\odot 2}\mathbf{1}_{k\times 1})^{\odot \frac{1}{2}}.
% \end{equation}
% \end{definition}

$\VCS$ will be added to $\VTR$, their labels are determined by $\YM^{(\text{base})}$

$\VUS$ will be sent LLMs for annotations.

The rest nodes in $\V\setminus \VTR$

\subsubsection{\bf Graph Rewiring}
GNNs are limited here due to noisy graph structure.

\begin{equation}
\HM = \textsf{Encoder}(\G, \YM^{(\text{base})})
\end{equation}

\begin{equation}
w(v_i,v_j) = \sigma(\HM_{i}\cdot\HM_{j}^{T})
\end{equation}
Here, \( \sigma \) is the ReLU function. 

\begin{equation}
\EDG_{\text{rm}} = \argtopk{(v_i,v_j)\in \EDG}{w(v_i,v_j)}
\end{equation}
\taiyan{Here $w(v_i,v_j)$ shouldn't be normalized like the way we choose the candidate edges, because $w(v_i,v_j)$ also works as the edge weight in the later computation. After normalization the value will approximate 0}
\begin{equation}
\EDG_{\text{ad}} = \argtopk{\substack{v_i\in \VTR, v_j\in \V\setminus\VTR\\ (v_i,v_i)\notin \EDG}}{w(v_i,v_j)}
\end{equation}

We create a rewired graph $\G_{\text{rw}}$ with edge set $(\EDG\cup \EDG_{\text{ad}})\setminus \EDG_{\text{rm}}$

\subsubsection{\bf Label Prediction and Loss Function}

\begin{equation}
\YM = \textsf{GNN}(\G_{\text{rw}}, \YM^{(\text{base})}),
\end{equation}

\begin{equation}
    \mathcal{L}_{\text{pred}} = \textsf{CrossEntropy}(\YM, \widehat{\YM})
\end{equation}

\begin{equation}
   \mathcal{L}_{\text{grw}} = \lambda_Y\cdot \Tr\left({\YM^{(\text{base})}}^\top \LM_{\text{rw}} \YM^{(\text{base})}\right) + \lambda_L\cdot \left\| \LM_{\text{rw}} \right\|^2_F 
\end{equation}

Dirichlet Energy, Tikhonov regularization~\cite{tikhonov1977solutions}

\subsubsection{\bf Label Correction for $\VUS$}

==> tex/pipeline_draft.tex <==
\eat{
\section{Methodology}

% \subsection{LM-based Text Embeddings}
% Use BERT or Sentence-BERT to get node initial embeddings

% \subsection{Graph Neural Networks}

% Use GNN to get node embeddings

% \subsection{Clustering Module}

% Use Embedding to get node-cluster indicator, i.e., centroid embeddings

\subsection{Data Preprocessing}

To begin, we employ an effective active learning method to obtain representative initial node labels. Suppose we need a total of \( \UM \) labeled nodes. To achieve this, we first augment the features with the graph topology by performing the following operation:

\begin{equation}
\ZM = \sum_{t=0}^{T}{\alpha^t \NAM^t \XM},
\end{equation}

where \( \NAM \) represents the normalized adjacency matrix, and \( \XM \) denotes the original node attribute matrix. This augmentation is the optimal solution to the Graph Laplacian Smoothing problem.

% To-do: add theoretical analysis (refer to Definition 3.1 in \url{https://arxiv.org/pdf/2403.13268}, Section 3.2 in \url{https://arxiv.org/pdf/2110.11842}, and Lemma 1 in \url{https://arxiv.org/pdf/2401.09071}).

Next, we apply a subspace clustering method, with the following objective function:

\begin{equation}
    \min_{\SM\in \mathbb{R}^{n\times n}} \left\{ \|\ZM - \SM \ZM\|_F^2 + \Omega(\SM) \right\},
\end{equation}

where \( \SM \) is the target self-representation or coefficient matrix, and \( \SM_{i,j} \) represents the affinity between nodes \( v_i \) and \( v_j \). Here, \( \SM = \UM \UM^{\top} \), where \( \UM \) consists of the top \( |\Sc| \) eigenvectors of \( \ZM \). Finally, we apply K-Means clustering on \( \UM \) to obtain \( |\Sc| \) centroids, denoted as \( \Sc \), representing the nodes selected for labeling.


After obtaining the K-means results, we refine the selection by choosing nodes that are closer to their respective cluster centers, as described in \cite{chen2023label}. This selection process is expressed as:

\begin{equation}
   v_i = \frac{1}{1 + \|\mathbf{u}_{v_i} - \mathbf{u}_{\text{CC}(v_i)}\|}
\end{equation}

where \( \mathbf{u}_{v_i} \) represents the decomposed feature of node \( v_i \), and \( \text{CC}(v_i) \) is the decomposed feature of the closest cluster center to node \( v_i \). \renchi{what does this mean? $v_i$ is a node. Why does the above equation assign a value to it? What is the purpose of computing this value?} \taiyan{This is the method used in LLMGNN\cite{chen2023label}, and it tend to select the nodes that most close to the cluster center. Here $u_{v_{i}}$ is the decomposed feature of node $v_{i}$ from $U$}

\subsection{Two-stage prompt}

Once the initial nodes are selected, the next step is to query the LLM to obtain the node labels. Inspired by the "cold start" and "warm start" concepts commonly used in recommendation systems, we propose a two-stage prompt method to achieve few-shot learning without any initial labels. The initial label selection is analogous to a cold start, where no prior information is available except for the label categories. Thus, we employ a zero-shot prompt to retrieve the labels and their associated confidence scores.

In this stage, we apply the zero-shot annotation with the consistency prompt strategy from \cite{chen2023label}, as shown below\ref{prompt:0_shot}:



The confidence scores are used to refine and filter out certain nodes in later stages of the process \cite{chen2023label}. Assuming the current selected set of nodes is denoted as \( \mathcal{V}_{\text{sel}} \), the Coefficient of Entropy (COE) can be computed as:

\begin{equation}
    \text{COE}(v_{i}) = \boldsymbol{H}(\Tilde{y}_{\mathcal{V}_{\text{sel}} \setminus \{v_{i}\}} ) - \boldsymbol{H}(\Tilde{y}_{\mathcal{V}_{\text{sel}}}),
\end{equation}

where \( \boldsymbol{H}() \) represents the Shannon entropy function, and \( \Tilde{y} \) refers to the annotations generated by LLMs. The final filtering score function, \( f_{\text{filter}} \), is defined as:

\begin{equation}
    f_{\text{filter}}(v_{i}) = \beta_{0} \times r_{f_{\text{conf}}(v_{i})} + \beta_{1} \times r_{\text{COE}(v_{i})},
\end{equation}

where hyperparameters \( \beta_{0} \) and \( \beta_{1} \) are introduced to balance between label diversity and annotation quality. Here, \( r_{f_{\text{conf}}} \) represents the ranking percentage (from high to low) of the confidence score \( f_{\text{conf}} \).

Once the initial nodes have been selected, we extract information from the LLM responses and incorporate this into the training-stage prompt, similar to the concept of a "warm start." For each label category, we select the most confident annotation as an example and include it in the training prompt. In some datasets, the label for a category may be a technical term that GPT-3.5 may not fully understand, so we also generate an explanation for each category. The full prompt for the training stage is as follows:\ref{prompt:c_shot}



Note that GPT-3.5 has a maximum input token limit of 16k tokens. If the total prompt, including all examples, exceeds this limit, the input may be truncated. To avoid this issue, we limit the token length of the example text. As the text length varies across different datasets, we fine-tune the token limit to ensure optimal performance within the input constraints.


\subsection{Training Pipeline}
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\textwidth/2]{pictures/structure.png}  
%     \caption{Algorithm Framework}
%     \label{fig:framework}
% \end{figure}

The overall training pipeline follows the framework illustrated in Figure \ref{fig:framework}. After obtaining the initial annotations, we first train a base GCN to compute the node representations as:

\begin{equation}
    Y_{\text{base}} = \text{GCN}(A, X),
\end{equation}

where \( Y_{\text{base}} \) is an \( N \times C \) matrix, and \( X \) represents the feature embeddings generated by Sentence-BERT \cite{chen2023label}. The predicted labels are obtained by computing \( \arg\max(Y_{\text{base}}) \). To select the nodes that require further annotation during training, we first introduce two key definitions.

\begin{definition}[Harmonicity]
\begin{equation}
\text{harmonicity} = \left( \left( \tilde{L}Y \right)^{\odot 2} \mathbf{1}_{c \times 1} \right)^{\odot \frac{1}{2}}
\end{equation}
Here, \( \tilde{\LM} = \IM - \DM^{-1}\AM \) is the random walk normalized Laplacian of graph \( \G \). This metric measures the smoothness of the graph structure, where a lower value indicates a smoother graph.
\end{definition}

\begin{definition}[Entropy]
\begin{equation}
\text{Entropy}(v) = -\sum_{\ell=1}^{k} \mathbf{Y}_{\ell} \cdot \log \left( \mathbf{Y}_{\ell} + \varepsilon \right)
\end{equation}
Here, \( \varepsilon \) is set to \( 1\text{e-9} \) to enhance stability. This entropy value quantifies the distribution of the final layer output \( Y^{n \times c} \) of the GCN. A higher value indicates a more uniform distribution.
\end{definition}

\subsubsection{Confidence-based Sample Selection}

Our goal is to select \( N_{\text{conf}} \) confident nodes and \( N_{\text{inconf}} \) unconfident nodes, and then incorporate their prediction results into the training set.

In general, the confidence of the model's predictions can be calculated by taking the index of the highest value from the output of the final layer, which we refer to as \textbf{raw confidence}. In practice, we observe that accuracy is positively correlated with confidence. However, high-confidence nodes may often come from a single cluster, leading to a lack of representativeness (e.g., selecting 40 nodes, with 35 nodes sharing the same label).

Given the aforementioned definitions, we propose a confident/inconfident node selection method, termed \textbf{smooth selection}. Suppose we have already computed the harmonicity and entropy for each node. In each stage, the selection rule is applied as follows:


\begin{equation}
\scalebox{0.8}{$
\{\text{Most\_Confident}\} = \left( \arg\min_{i \in \text{N}_{\text{unlabel}}}^{N_{\text{conf}}} \left( \text{Harm}(\mathbf{Y}, \mathbf{E}) \right) \cap \arg\min_{i \in \text{N}_{\text{unlabel}}}^{N_{\text{conf}}} \left( H(\mathbf{Y}) \right) \right)
$}
\end{equation}

\begin{equation}
\scalebox{0.8}{$
\{\text{Most\_Inconfident}\} = \left( \arg\max_{i \in N_{\text{unlabel}}}^{N_{\text{inconf}}} \left( \text{Harm}(\mathbf{Y}, \mathbf{E}) \right) \cap \arg\max_{i \in N_{\text{unlabel}}}^{N_{\text{inconf}}} \left( H(\mathbf{Y}) \right) \right)
$}
\end{equation}

\begin{equation}
\scalebox{0.8}{$
\{\text{Confident}\} = \left( \arg\min_{i \in N_{\text{unlabel}}}^{N_{\text{conf}}} \left( \text{Harm}(\mathbf{Y}, \mathbf{E}) \right) \cup \arg\min_{i \in N_{\text{unlabel}}}^{N_{\text{conf}}} \left( H(\mathbf{Y}) \right) \right) \setminus \{\text{Most\_Confident}\}
$}
\end{equation}

\begin{equation}
\scalebox{0.8}{$
\{\text{Inconfident}\} = \left( \arg\max_{i \in N_{\text{unlabel}}}^{N_{\text{inconf}}} \left( \text{Harm}(\mathbf{Y}, \mathbf{E}) \right) \cup \arg\max_{i \in N_{\text{unlabel}}}^{N_{\text{inconf}}} \left( H(\mathbf{Y}) \right) \right) \setminus \{\text{Most\_Inconfident}\}
$}
\end{equation}

\begin{equation}
\scalebox{0.8}{$
\{\text{Final\_Most\_Confident\_Set}\} = \{\text{Most\_Confident}\} \cup \binom{\left| \text{Confident} \right|}{N_{\text{conf}} - |\text{Most\_Confident}|}
$}
\end{equation}

\begin{equation}
\scalebox{0.8}{$
\{\text{Final\_Most\_Inconfident\_Set}\} = \{\text{Most\_Inconfident}\} \cup \binom{\left| \text{Inconfident} \right|}{N_{\text{inconf}}-|\text{Most\_Inconfident}|}
$}
\end{equation}
Here, $H$ represents the label entropy, while $Harm$ refers to the harmonicity measure.

In practice, although this selection metric can improve the model's upper bound by selecting more representative nodes, we observe that the accuracy of the selected nodes may sometimes be lower than those selected based on raw confidence. Lower accuracy introduces more noise into the label annotation process. Therefore, we propose a hybrid selection method, combining smooth selection to obtain confident samples and raw confidence selection to identify inconfident samples. \renchi{unclear. What we will do to these selected nodes?} \taiyan{[Select confident nodes by the above equation, inconfident nodes by $\arg\max(\text({raw\_confident})$]}

\subsubsection{Label Correction}

Due to the complexity and noise present in text-attributed graphs and the limited comprehension capabilities of large language models (LLMs), the responses from LLMs can be quite noisy. LLMs only consider node attributes as input, while graph neural networks (GNNs) take both graph topology and node features into account. This difference may result in significant deviations in prediction results. In the sample selection process, our goal is to identify low-accuracy nodes from GNN predictions and use LLMs to correct them. Simultaneously, we can leverage GNNs to correct noisy LLM responses interactively. Based on this idea, we designed the label correction module.

Our label correction module consists of two components: an edge predictor and a node predictor. Inspired by \cite{dai2021nrgnnlearninglabelnoiseresistant}, we first optimize the connections between currently annotated nodes and unannotated nodes. After this step, we obtain an updated graph structure. This updated graph, along with the annotations from the initial and previously selected samples, is then used to train a GNN. The GNN predictions are subsequently employed to correct the LLM annotations.

To train a model that produces a more accurate graph structure, we minimize the \textit{Dirichlet Energy} of the graph. To prevent the degree distribution of the graph from becoming too imbalanced, we also incorporate a penalty term into the objective function. The minimization objective can be formulated as:

\begin{equation}
    \min( \alpha \times \text{tr}(Y^T L Y) + \beta \times \left\| L \right\|^2 )
\end{equation}

Here, $Y$ is the feature matrix, $L = D - A$ represents the graph Laplacian, and $\left\| L \right\|$ denotes the Frobenius norm. This objective serves as a measure of the graph's smoothness, where a lower value indicates a smoother graph. Since typical GCN models and their variants operate under a homophily assumption, a smoother graph is easier for GCNs and their variants to predict.

In our practice, we train a GCN to minimize the loss function. The output of the GCN is as follows:

\begin{equation}
    Y_{e} = \text{MLP}(Y_{\text{base}})
\end{equation}

 Here the activate function is SReLU\cite{jin2015deeplearningsshapedrectified}. A detailed explanation of why we use SReLU can be found in the appendix.It is important to note that our smoothing process is based on the output of the base GCN, rather than the original feature matrix \( X \). Suppose \( e_i \) and \( e_j \) represent the node embeddings for nodes \( v_i \) and \( v_j \), respectively. The similarity between these two nodes is computed as:

\begin{equation}
    S_{ij} = \sigma(e_{i} e_{j}^{T})
\end{equation}

Here, \( \sigma \) is the ReLU function. Given that a graph may contain up to \( N \times N \) edges, it is computationally infeasible to calculate the similarity between every pair of nodes and then select nodes for rewiring. Therefore, we first select candidate edges based on the following rule: \textit{Only consider the connections between labeled nodes and unlabeled nodes. For each unlabeled node, consider only the top \( M \) most similar labeled nodes.} Here, \( M \) is a tunable parameter and is no larger than the size of the labeled node set.

Suppose the labeled node set is denoted as \( N_{\text{label}} \) and the unlabeled node set as \( N_{\text{unlabel}} \). The similarity between a labeled node \( i \) and an unlabeled node \( j \) can be expressed as: \renchi{what are \( N_{\text{label}} \) and \( N_{\text{unlabel}} \)?} \taiyan{Here  \( N_{\text{label}} \) and \( N_{\text{unlabel}} \) is the labeled node set and unlabeled node set, the same as train set and test set}

\begin{equation}
    \text{sim}(i, j) = \frac{\mathbf{e}_i \cdot \mathbf{e}_j}{\|\mathbf{e}_i\| \|\mathbf{e}_j\|}, \quad \text{for } i \in N_{\text{label}}, j \in N_{\text{unlabel}}
\end{equation}

For each unlabeled node \( j \), we select the top \( M \) most similar labeled nodes as follows:

\begin{equation}
    \text{Top}_M(j) = \arg\max_{i \in N_{\text{label}}} \left( \text{sim}(i, j) \right), \quad i \in \{1, 2, \dots, |N_{\text{label}}|\}
\end{equation}


The set of candidate edges \( P_e \) is then defined as:

\begin{equation}
    P_e = \left\{ (i, j) \mid i \in \text{Top}_M(j) \text{ and } (i, j) \notin E \right\}
\end{equation}


Then we change the graph structure with the candidate edge set $P_{e}$. First, we set a change ratio $C_{r}$ and change interval $C_{i}$, which means every $C_{i}$ epoch, $C_{r}\times |E|$ edges will be changed. Suppose we have the edge predictor's $Y_e$ and the similarity score $S_{orig}, S_{candidate}$ of the current graph edges and candidate edges, the structure adjustment can be expressed by \renchi{How to use $P_{e}$?}
\taiyan{my mistake. below 'candidate' should be $P_e$}
\begin{equation}
\mathbf{E}_{\text{remove}} = \arg\min \left( \mathbf{S}_{\text{orig}}^{ \left( |\mathbf{E}_{\text{orig}}| \times C_{\text{r}} \right)} \right)
\end{equation}
\begin{equation}
\mathbf{E}_{\text{add}} = \arg\max \left( \mathbf{S}_{P_e}^{\left( |\mathbf{E}_{\text{orig}}| \times C_{\text{r}} \right)} \right)
\end{equation}
\begin{equation}
\mathbf{E}_{\text{new}} = \left( \mathbf{E}_{\text{orig}} \setminus \mathbf{E}_{\text{remove}} \right) \cup \mathbf{E}_{\text{add}}
\end{equation}
This selection method ensures that at each update stage $C_i$, the most dissimilar edges are deleted, and the most similar edges are added. Then with the updated graph, we train another GCN to examine the effect of the GCN work on the updated graph by predicting the node label. The prediction works as
\begin{equation}
    \hat{Y}^{P} = GCN(E_{new}, Y_{base}, S_{new})
\end{equation}
Where $E_{new}$ is the updated graph structure, $Y_{base}$ is the output embedding of the base GCN, and $S_{new}$ is the node pair similarity, and here we take it as the edge weight. 
% \begin{equation}
% \mathcal{L}_{\text{total}} = \mathcal{L}_{\text{pred}} + \mathcal{L}_{\text{rec}}
% \end{equation}
% Where
\begin{equation}
    \mathcal{L}_{\text{pred}} = \text{CrossEntropy}(\hat{y}_{p}, y)
\end{equation}
\begin{equation}
   \mathcal{L}_{\text{rec}} = \alpha \times \text{tr}(Y_{base}^T L Y_{base}) + \beta \times \left\| L \right\|^2 
\end{equation}
\subsubsection{Post Correction}

In this module, we use the label corrector's prediction \( \arg\max \hat{Y}^{p} \) to correct the LLM annotations. Similar to the selection method described in \textit{Section 4.3.1}, we apply the following strategy to  correct the LLM annotations:

\begin{align}
\text{if } &\left( r_{f_{\text{conf}}(v_{i})} < r_{\hat{Y}_{p}(i)} \right) \\
&\text{or } f_{\text{conf}}(v_{i}) < \text{LLM\_score\_threshold} \\
&\text{then } y_i = \hat{y}_i
\end{align}

Here, \( \text{LLM\_score\_threshold} \) is a threshold value we set, and \( r \) indicates the rank within the selected node set \renchi{what is the selected node set?}. \renchi{when we do this?}
\taiyan{In the figure\ref{fig:framework} Post Selection part. these selected nodes are the pseudo labels we select and put to the next stage's training}

}

\eat{
\subsubsection{N-Stage Self-Training}

We repeat the entire pipeline \( N \) times to gradually integrate pseudo labels and annotated labels into the labeled set \( N_{\text{label}} \). This self-training strategy has been widely adopted in previous works \cite{liu2022confidencecheatselftraininggraph}\cite{article}. However, previous approaches relied solely on their own model's knowledge, which can introduce bias and noise. To the best of our knowledge, we are the first to incorporate LLM queries into the GNN self-training process.
}



